The HeRSCheL detector: high-rapidity shower counters for LHCb

The HeRSCheL detector consists of a set of scintillating counters, designed to increase the coverage of the LHCb experiment in the high-rapidity regions on either side of the main spectrometer. The new detector improves the capabilities of LHCb for studies of diffractive interactions, most notably Central Exclusive Production. In this paper the construction, installation, commissioning, and performance of HeRSCheL are presented.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 

